VisDA-2021 Competition Universal Domain Adaptation to Improve Performance on Out-of-Distribution Data

Progress in machine learning is typically measured by training and testing a model on the same distribution of data, i.e., the same domain. This over-estimates future accuracy on out-of-distribution data. The Visual Domain Adaptation (VisDA) 2021 competition tests models' ability to adapt to novel test distributions and handle distributional shift. We set up unsupervised domain adaptation challenges for image classifiers and will evaluate adaptation to novel viewpoints, backgrounds, modalities and degradation in quality. Our challenge draws on large-scale publicly available datasets but constructs the evaluation across domains, rather that the traditional in-domain bench-marking. Furthermore, we focus on the difficult "universal" setting where, in addition to input distribution drift, methods may encounter missing and/or novel classes in the target dataset. Performance will be measured using a rigorous protocol, comparing to state-of-the-art domain adaptation methods with the help of established metrics. We believe that the competition will encourage further improvement in machine learning methods' ability to handle realistic data in many deployment scenarios.

==> office_dance.tex <==
\begin{table}[t]
 \addtolength{\tabcolsep}{-3pt}
\begin{center}
\scalebox{1.0}{

\begin{tabular}{l|cccccc|c}
\toprule[1.5pt]
\multirow{2}{*}{Method}& \multicolumn{6}{c|}{Office}&\multirow{2}{*}{Avg}\\
     & A2D  & A2W  & D2A  & D2W  & W2D  & W2A  &   \\\hline
UAN~\cite{UDA_2019_CVPR}          & 59.7 & 58.6 & 60.1 & 70.6 & 71.4 & 60.3 & 63.5 \\
CMU~\cite{fu2020learning}          & 68.1 & 67.3 & 71.4 & 79.3 & 80.4 & 72.2 & 73.1 \\
DANCE~\cite{saito2020universal}	&78.6&71.5&79.9&91.4&87.9&72.2&80.3 \\
  \bottomrule[1.5pt]
\end{tabular}}
\end{center}
\vspace{-7mm}
\caption{\small \textbf{H-score of open-partial domain adaptation using Office (higher is better)}, where 10 shared classes, 10 source-private classes, and 11 target private classes are used. Each column shows the results of different adaptation scenarios, e.g., A2D is the shift from ``Amazon" to ``DSLR".}
\label{tb:office_opda}

\end{table}
